Towards Efficient Anytime Computation and Execution of Decoupled Robustness Envelopes for Temporal Plans

One of the major limitations for the employment of model-based planning and scheduling in practical applications is the need of costly re-planning when an incongruence between the observed reality and the formal model is encountered during execution. Robustness Envelopes characterize the set of possible contingencies that a plan is able to address without re-planning, but their exact computation is extremely expensive; furthermore, general robustness envelopes are not amenable for efficient execution. In this paper, we present a novel, anytime algorithm to approximate Robustness Envelopes, making them scalable and executable. This is proven by an experimental analysis showing the efficiency of the algorithm, and by a concrete case study where the execution of robustness envelopes significantly reduces the number of re-plannings.

==> tricks.tex <==
% \renewcommand{\baselinestretch}{0.987}
% \setlength\titlebox{1.7in}

% \setlength\dbltextfloatsep{2pt}
% \setlength{\floatsep}{4pt}
%\setlength\textfloatsep{8pt}

% \setlength{\abovecaptionskip}{5pt plus 3pt minus 2pt}
% \setlength{\belowcaptionskip}{5pt plus 3pt minus 2pt}

%% \makeatletter
%% \g@addto@macro\normalsize{%
%%   \setlength\abovedisplayskip{5pt}
%%   \setlength\belowdisplayskip{5pt}
%%   \setlength\abovedisplayshortskip{5pt}
%%   \setlength\belowdisplayshortskip{5pt}
%% }
%% \makeatother

